Busca de melhor caminho entre m\'ultiplas origens e m\'ultiplos destinos em redes complexas que representam cidades

Was investigated in this paper the use of a search strategy in the problem of finding the best path among multiple origins and multiple destinations. In this kind of problem, it must be decided within a lot of combinations which is the best origin and the best destination, and also the best path between these two regions. One remarkable difficulty to answer this sort of problem is to perform the search in a reduced time. This monography is a extension of previous research in which the problem described here was studied only in a bus network in the city of Fortaleza. This extension consisted of an exploration of the search strategy in graphs that represent public ways in cities like Fortaleza, Mumbai and Tokyo. Using this strategy with a heuristic algorithm, Haversine distance, was noticed that is possible to reduce substantially the time of the search, but introducing an error because of the loss of the admissible characteristic of the heuristic function applied.

==> elementos-pos-textuais/apendices/termo-de-fiel-depositario.tex <==
% \apendice{Termo de Fiel Depositário}
% \label{ap:termo-de-fiel-depositario}

% \noindent \textbf{Pesquisa:} ANÁLISE DA MORTALIDADE INFANTIL COM MALFORMAÇÕES CONGÊNITAS.

% \noindent Pelo presente instrumento que atende às exigências legais, a Sra. Maria Consuelo Martins Saraiva, ``fiel depositário'' com o cargo de Secretária Municipal de Saúde de Iracema, após ter tomado conhecimento do protocolo de pesquisa intitulado: ANÁLISE DA MORTALIDADE INFANTIL COM MALFORMAÇÕES CONGÊNITAS. Analisando a repercussão desse estudo no contexto da saúde pública e epidemiologia, autoriza Karla Maria da Silva Lima, enfermeira, aluna do Curso de Mestrado Acadêmico em Enfermagem da Universidade Estadual do Ceará (UECE), sob orientação do Prof. Dr. José Maria de Castro, da UECE, ter acesso aos bancos de dados do Sistema de Informação sobre Nascidos Vivos e do Sistema de Informação sobre Mortalidade da Secretaria Municipal de Saúde de Iracema, objeto deste estudo, e que se encontram sob sua total responsabilidade. Fica claro que o Fiel Depositário pode a qualquer momento retirar sua AUTORIZAÇÃO e ciente de que todas as informações prestadas tornar-se-ão confidenciais e guardadas por força de sigilo profissional, assegurando que os dados obtidos da pesquisa serão somente utilizados para estudo.

==> elementos-pos-textuais/glossario.tex <==
% \newglossaryentry{ambiguidade}{
% 	name=Ambiguidade,
% 	description={possibilidade de interpretação dúbia de uma palavra ou frase}
% }

% \newglossaryentry{braile}{
% 	name=Braile,
% 	description={sistema de escrita para cegos. São signos desenhados em relevo para serem lidos com a ponta dos dedos}
% }

% \newglossaryentry{borboleta}{
% 	name=Borboleta,
% 	description={inseto voador, que possui dois pares de asas. São todos os insetos alados da família dos lepidópteros diurnos. São encontrada na natureza com diversas cores e tamanho}
% }

% \newglossaryentry{coerencia}{
% 	name=Coerência,
% 	description={qualidade subjacente a um texto, que lhe permite ter sentido}
% }

% \newglossaryentry{dialetos}{
% 	name=Dialetos,
% 	description={variedades regionais ou sociais de uma língua}
% }

% \newglossaryentry{elipse}{
% 	name=Elipse,
% 	description={omissão de termos da oração}
% }

% \newglossaryentry{locucao-adjetiva}{
% 	name=Locução Adjetiva,
% 	description={duas ou mais palavras que equivalem a um adjetivo}
% }

% \newglossaryentry{modificadores}{
% 	name=Modificadores,
% 	description={adjetivos}
% }

% \newglossaryentry{paronimos}{
% 	name=Parônimos,
% 	description={palavras que possuem sons parecidos. Exemplo: emigrar / imigrar}
% }

% \newglossaryentry{sintese}{
% 	name=Síntese,
% 	description={exposição resumida, em que se usa um mínimo de palavras}
% }





==> elementos-pre-textuais/agradecimentos.tex <==
% Primeiramente a Deus que permitiu que tudo isso acontecesse, ao longo de minha vida, e não somente nestes anos como universitária, mas que em todos os momentos é o maior mestre que alguém pode conhecer.
	
% Aos meus pais, pelo amor, incentivo e apoio incondicional.

% Obrigada meus irmãos e sobrinhos, que nos momentos de minha ausência dedicados ao estudo superior, sempre fizeram entender que o futuro é feito a partir da constante dedicação no presente!

% A esta universidade, seu corpo docente, direção e administração que oportunizaram a janela que hoje vislumbro um horizonte superior, eivado pela acendrada confiança no mérito e ética aqui presentes.

% Agradeço a todos os professores por me proporcionar o conhecimento não apenas racional, mas a manifestação do caráter e afetividade da educação no processo de formação profissional, por tanto que se dedicaram a mim, não somente por terem me ensinado, mas por terem me feito aprender. a palavra mestre, nunca fará justiça aos professores dedicados aos quais sem nominar terão os meus eternos agradecimentos.

==> elementos-pre-textuais/dedicatoria.tex <==
% Este trabalho é dedicado às crianças adultas que, quando pequenas, sonharam em se tornar cientistas.

==> elementos-pre-textuais/epigrafe.tex <==
% ``É melhor lançar-se à luta em busca do triunfo mesmo expondo-se ao insucesso, que formar fila com os pobres de espírito, que nem gozam muito nem sofrem muito; E vivem nessa penumbra cinzenta sem conhecer nem vitoria nem derrota.''

% \autordaepigrafe{Franklin Roosevelt}

% % Deixe o espaço entre a epigrafe e o autor.

==> elementos-pre-textuais/errata.tex <==
% Elemento opcional da \cite[4.2.1.2]{NBR14724:2011}. Exemplo:

% \vspace{\onelineskip}

% FERRIGNO, C. R. A. \textbf{Tratamento de neoplasias ósseas apendiculares com
% 	reimplantação de enxerto ósseo autólogo autoclavado associado ao plasma
% 	rico em plaquetas}: estudo crítico na cirurgia de preservação de membro em
% cães. 2011. 128 f. Tese (Livre-Docência) - Faculdade de Medicina Veterinária e
% Zootecnia, Universidade de São Paulo, São Paulo, 2011.

% \begin{table}[htb]
% 	\center
% 	\footnotesize
% 	\begin{tabular}{|p{1.4cm}|p{1cm}|p{3cm}|p{3cm}|}
% 		\hline
% 		\textbf{Folha} & \textbf{Linha}  & \textbf{Onde se lê}  & \textbf{Leia-se}  \\
% 		\hline
% 		1 & 10 & auto-conclavo & autoconclavo\\
% 		\hline
% 	\end{tabular}
% \end{table}


==> elementos-pre-textuais/lista-de-abreviaturas-e-siglas.tex <==
% \newacronym{TMMFC}{TMMFC}{Taxa de Mortalidade por Malformação Congênita}
% \newacronym{TMI}{TMI}{Taxa de Mortalidade Infantil}
% \newacronym{SUS}{SUS}{Sistema Único de Saúde}
% \newacronym{DO}{DO}{Declaração de Óbito}
% \newacronym{DNV}{DNV}{Declaração de Nascido Vivo}
% \newacronym{PNI}{PNI}{Programa Nacional de Imunização}
% \newacronym{ONU}{ONU}{Organização das Nações Unidades}
% \newacronym{OMS}{OMS}{Organização Mundial de Saúde}
% \newacronym{SINASC}{SINASC}{Sistema de Informação de Nascidos Vivos}
% \newacronym{SIM}{SIM}{Sistema de Informação de Mortalidade}
% \newacronym{RN}{RN}{Recém-nascido}
% \newacronym{MS}{MS}{Ministério da Saúde}
% \newacronym{MI}{MI}{Mortalidade Infantil}
% \newacronym{MFC}{MFC}{Malformação Congênita}
% \newacronym{OI}{OI}{Óbito Infantil}
% \newacronym{ODM}{ODM}{Objetivos do Desenvolvimento do Milênio}
% \newacronym{NV}{NV}{Nascido Vivo}
% \newacronym{IBGE}{IBGE}{Instituto Brasileiro de Geografia e Estatística}
% \newacronym{ESF}{ESF}{Estratégia de Saúde da Família}
% \newacronym{DATASUS}{DATASUS}{Departamento de Informática do Sistema Único de Saúde}
% \newacronym{RIPSA}{RIPSA}{Rede Interagencial de Informações para a Saúde}
% \newacronym{PSF}{PSF}{Programa Saúde da Família}
\newacronym{API}{API}{Application Programming Interface}
\newacronym{XML}{XML}{Extensible Markup Language}
\newacronym{OD}{OD}{Origem e Destino}
\newacronym{MOMD}{MOMD}{Múltiplas Origens e Múltiplos Destinos}



==> elementos-pre-textuais/lista-de-simbolos.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%   Atencao! A lista nao ordena automaticamente   %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{simbolos} \itemsep -1pt
% 	\item[$ Ae $] Área efetiva da antena
% 	\item[$ B $] Largura de faixa em que o ruído é medido em Hertz
% 	\item[$ d $] Distância em metros
% 	\item[$ E $] Campo elétrico
% 	\item[$ FA $] Fator da antena
% 	\item[$ Gr $] Ganho de recepção
% 	\item[$ h $] Altura efetiva ou comprimento efetivo de uma antena
% 	\item[$ I $] Corrente elétrica
% 	\item[$ k $] Constante de Boltzmann’s
% 	\item[$ K $] Eficiência de irradiação
% 	\item[$ M $] Variação do patamar de ruído em função da RBW
% 	\item[$ N $] Condutor de neutro
% 	\item[$ NF $] Figura de ruído
% 	\item[$ Ni $] Potência do ruído na entrada
% 	\item[$ No $] Potência do ruído na saída
% 	\item[$ P $] Potência
% 	\item[$ R $] Resistência
% 	\item[$ Si $] Potência do sinal na entrada
% 	\item[$ So $] Potência do sinal na saída
% 	\item[$ t $] Tempo
% 	\item[$ V $] Tensão
% 	\item[$ ZL  $] Impedância da antena
% 	\item[$ Zo $] Impedância de referência (50$\Omega$)
% 	\item[$ \lambda $] Comprimento de onda 
% 	\item[$ \Gamma $] Coeficiente de reflexão	
% \end{simbolos}
